CRADLE-VAE: Enhancing Single-Cell Gene Perturbation Modeling with Counterfactual Reasoning-based Artifact Disentanglement

Predicting cellular responses to various perturbations is a critical focus in drug discovery and personalized therapeutics, with deep learning models playing a significant role in this endeavor. Single-cell datasets contain technical artifacts that may hinder the predictability of such models, which poses quality control issues highly regarded in this area. To address this, we propose CRADLE-VAE, a causal generative framework tailored for single-cell gene perturbation modeling, enhanced with counterfactual reasoning-based artifact disentanglement. Throughout training, CRADLE-VAE models the underlying latent distribution of technical artifacts and perturbation effects present in single-cell datasets. It employs counterfactual reasoning to effectively disentangle such artifacts by modulating the latent basal spaces and learns robust features for generating cellular response data with improved quality. Experimental results demonstrate that this approach improves not only treatment effect estimation performance but also generative quality as well. The CRADLE-VAE codebase is publicly available at https://github.com/dmis-lab/CRADLE-VAE.

==> tables/table4_results2.tex <==
\begin{table*}[hbt!]
{\large
\resizebox*{\textwidth}{!}{%
\renewcommand{\arraystretch}{1.4}
% Please add the following required packages to your document preamble:
% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
\begin{tabular}{cl|cccc|llll}
\hline
\multicolumn{2}{c|}{\textbf{Dataset}}                                                                                         & \multicolumn{4}{c|}{\textbf{Replogle}}                                                                                                                                                                         & \multicolumn{4}{c}{\textbf{Adamson}}                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{c|}{Model}                     & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}QC \\ threshold\end{tabular}} & \begin{tabular}[c]{@{}c@{}}ATE-\\ pearson\end{tabular} & ATE-r2                                       & Jaccard                                      & \begin{tabular}[c]{@{}c@{}}QC pass \\ rate\end{tabular} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}ATE-\\ pearson\end{tabular}} & \multicolumn{1}{c}{ATE-r2}                   & \multicolumn{1}{c}{Jaccard}                  & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}QC pass \\ rate\end{tabular}} \\ \hline
\multicolumn{1}{c|}{Conditional VAE}           &                                                                              & {\underline {0.7022\scriptsize ± 0.00\normalsize}}              & {\underline {0.4883\scriptsize ± 0.01\normalsize}}    & \textbf{0.2688\scriptsize ± 0.00\normalsize} & {\underline {76.56\scriptsize ± 0.26\normalsize}}                & {\underline {0.6335\scriptsize ± 0.01\normalsize}}                                  & {\underline {0.3954\scriptsize ± 0.01\normalsize}}    & {\underline {0.3110\scriptsize ± 0.01\normalsize}}    & 77.23\scriptsize ± 0.44\normalsize                                          \\
\multicolumn{1}{c|}{CPA-VAE}                   &                                                                              & 0.5171\scriptsize ± 0.01\normalsize                    & 0.1241\scriptsize ± 0.02\normalsize          & 0.1438\scriptsize ± 0.00\normalsize          & 74.83\scriptsize ± 0.50\normalsize                      & 0.5571\scriptsize ± 0.02\normalsize                                        & 0.2637\scriptsize ± 0.03\normalsize          & 0.2123\scriptsize ± 0.01\normalsize          & 76.64\scriptsize ± 0.90\normalsize                                          \\
\multicolumn{1}{c|}{sVAE+}                     & \multicolumn{1}{c|}{$3\sigma$}                                               & 0.5780\scriptsize ± 0.01\normalsize                    & 0.3222\scriptsize ± 0.01\normalsize          & 0.1565\scriptsize ± 0.00\normalsize          & 73.89\scriptsize ± 0.53\normalsize                      & 0.5298\scriptsize ± 0.02\normalsize                                        & 0.2580\scriptsize ± 0.03\normalsize          & 0.1778\scriptsize ± 0.01\normalsize          & 76.27\scriptsize ± 0.98\normalsize                                          \\
\multicolumn{1}{c|}{SAMS-VAE}                  &                                                                              & 0.6798\scriptsize ± 0.03\normalsize                    & 0.4584\scriptsize ± 0.04\normalsize          & 0.2404\scriptsize ± 0.02\normalsize          & 74.96\scriptsize ± 0.69\normalsize                      & 0.3901\scriptsize ± 0.01\normalsize                                        & 0.1432\scriptsize ± 0.01\normalsize          & 0.1846\scriptsize ± 0.01\normalsize          & {\underline {77.34\scriptsize ± 0.78\normalsize}}                                    \\
\multicolumn{1}{c|}{\modelname (QC $3\sigma$)} &                                                                              & \textbf{0.7192\scriptsize ± 0.01\normalsize}           & \textbf{0.5155\scriptsize ± 0.01\normalsize} & {\underline {0.2667\scriptsize ± 0.01\normalsize}}    & \textbf{97.33\scriptsize ± 0.04\normalsize}             & \textbf{0.7529\scriptsize ± 0.01\normalsize}                               & \textbf{0.5611\scriptsize ± 0.02\normalsize} & \textbf{0.3471\scriptsize ± 0.01\normalsize} & \textbf{89.92\scriptsize ± 0.47\normalsize}                                 \\ \hline
\multicolumn{1}{c|}{Conditional VAE}           &                                                                              & {\underline {0.7255\scriptsize ± 0.01\normalsize}}              & {\underline {0.5233\scriptsize ± 0.01\normalsize}}    & {\underline {0.2776\scriptsize ± 0.00\normalsize}}    & {\underline {84.36\scriptsize ± 0.24\normalsize}}                & {\underline {0.6435\scriptsize ± 0.01\normalsize}}                                  & {\underline {0.4059\scriptsize ± 0.02\normalsize}}    & {\underline {0.3109\scriptsize ± 0.01\normalsize}}    & 85.06\scriptsize ± 0.52\normalsize                                          \\
\multicolumn{1}{c|}{CPA-VAE}                   &                                                                              & 0.5352\scriptsize ± 0.01\normalsize                    & 0.1765\scriptsize ± 0.03\normalsize          & 0.1494\scriptsize ± 0.01\normalsize          & 82.92\scriptsize ± 0.38\normalsize                      & 0.5715\scriptsize ± 0.02\normalsize                                        & 0.2863\scriptsize ± 0.03\normalsize          & 0.2103\scriptsize ± 0.01\normalsize          & 84.80\scriptsize ± 0.67\normalsize                                          \\
\multicolumn{1}{c|}{sVAE+}                     & \multicolumn{1}{c|}{$4\sigma$}                                               & 0.6056\scriptsize ± 0.01\normalsize                    & 0.3612\scriptsize ± 0.01\normalsize          & 0.1661\scriptsize ± 0.00\normalsize          & 82.15\scriptsize ± 0.50\normalsize                      & 0.5437\scriptsize ± 0.02\normalsize                                        & 0.2774\scriptsize ± 0.03\normalsize          & 0.1773\scriptsize ± 0.01\normalsize          & 84.66\scriptsize ± 0.60\normalsize                                          \\
\multicolumn{1}{c|}{SAMS-VAE}                  &                                                                              & 0.7086\scriptsize ± 0.03\normalsize                    & 0.4941\scriptsize ± 0.04\normalsize          & 0.2516\scriptsize ± 0.02\normalsize          & 83.01\scriptsize ± 0.43\normalsize                      & 0.3939\scriptsize ± 0.01\normalsize                                        & 0.1442\scriptsize ± 0.01\normalsize          & 0.1808\scriptsize ± 0.01\normalsize          & {\underline {85.36\scriptsize ± 0.75\normalsize}}                                    \\
\multicolumn{1}{c|}{\modelname (QC $4\sigma$)} &                                                                              & \textbf{0.7565\scriptsize ± 0.01\normalsize}           & \textbf{0.5595\scriptsize ± 0.01\normalsize} & \textbf{0.2869\scriptsize ± 0.01\normalsize} & \textbf{98.10\scriptsize ± 0.18\normalsize}             & \textbf{0.7636\scriptsize ± 0.01\normalsize}                               & \textbf{0.5770\scriptsize ± 0.01\normalsize} & \textbf{0.3367\scriptsize ± 0.01\normalsize} & \textbf{93.66\scriptsize ± 0.56\normalsize}                                 \\ \hline
\multicolumn{1}{c|}{Conditional VAE}           &                                                                              & {\underline {0.7296\scriptsize ± 0.01\normalsize}}              & {\underline {0.5282\scriptsize ± 0.01\normalsize}}    & {\underline {0.2793\scriptsize ± 0.00\normalsize}}    & {\underline {88.45\scriptsize ± 0.27\normalsize}}                & {\underline {0.6484\scriptsize ± 0.01\normalsize}}                                  & {\underline {0.4110\scriptsize ± 0.02\normalsize}}    & {\underline {0.3110\scriptsize ± 0.01\normalsize}}    & 88.75\scriptsize ± 0.45\normalsize                                          \\
\multicolumn{1}{c|}{CPA-VAE}                   &                                                                              & 0.5380\scriptsize ± 0.02\normalsize                    & 0.1999\scriptsize ± 0.03\normalsize          & 0.1501\scriptsize ± 0.01\normalsize          & 87.20\scriptsize ± 0.38\normalsize                      & 0.5758\scriptsize ± 0.02\normalsize                                        & 0.2928\scriptsize ± 0.04\normalsize          & 0.2102\scriptsize ± 0.01\normalsize          & 88.34\scriptsize ± 0.57\normalsize                                          \\
\multicolumn{1}{c|}{sVAE+}                     & \multicolumn{1}{c|}{$5\sigma$}                                               & 0.6137\scriptsize ± 0.01\normalsize                    & 0.3736\scriptsize ± 0.01\normalsize          & 0.1694\scriptsize ± 0.00\normalsize          & 86.60\scriptsize ± 0.41\normalsize                      & 0.5488\scriptsize ± 0.02\normalsize                                        & 0.2843\scriptsize ± 0.03\normalsize          & 0.1776\scriptsize ± 0.01\normalsize          & 88.65\scriptsize ± 0.55\normalsize                                          \\
\multicolumn{1}{c|}{SAMS-VAE}                  &                                                                              & 0.7167\scriptsize ± 0.03\normalsize                    & 0.4998\scriptsize ± 0.03\normalsize          & 0.2558\scriptsize ± 0.02\normalsize          & 87.26\scriptsize ± 0.33\normalsize                      & 0.3952\scriptsize ± 0.01\normalsize                                        & 0.1442\scriptsize ± 0.01\normalsize          & 0.1792\scriptsize ± 0.01\normalsize          & {\underline {89.05\scriptsize ± 0.49\normalsize}}                                    \\
\multicolumn{1}{c|}{\modelname (QC $5\sigma$)} &                                                                              & \textbf{0.7638\scriptsize ± 0.01\normalsize}           & \textbf{0.5719\scriptsize ± 0.01\normalsize} & \textbf{0.2931\scriptsize ± 0.01\normalsize} & \textbf{98.41\scriptsize ± 0.13\normalsize}             & \textbf{0.7609\scriptsize ± 0.01\normalsize}                               & \textbf{0.5723\scriptsize ± 0.01\normalsize} & \textbf{0.3153\scriptsize ± 0.00\normalsize} & \textbf{94.34\scriptsize ± 0.42\normalsize}                                 \\ \hline
\end{tabular}
}
\captionsetup{justification=raggedright, singlelinecheck=false}
\caption{Quantitative evaluation on Dixit dataset and Frangieh dataset across ${3\sigma, 4\sigma, 5\sigma}$ quality control (QC) thresholds. Note that the 'QC threshold' column refers to the cut-off point -- defined as delta-MAD threshold -- of the generated data to be included in the evaluation phase.}
}
\label{tab:notused_results}
\end{table*}

==> tables/table_qc_metric.tex <==
%table_qc_metric

\begin{table}[hbt!]
{\huge
\resizebox*{0.5\columnwidth}{!}{%
\renewcommand{\arraystretch}{1.4}
\begin{tabular}{cccc}
\toprule[2pt]
\textbf{QC Metric}      & \textbf{Cut-off} $(\sigma)$     & \textbf{sample ratio}     & \textbf{Reference} 
\\ \hline
number of UMI           & 3 / 4 / 5                & 30 / 1000     & ~\cite{you2021benchmarking, ocasio2019scrna}
\\
number of features      & 3 / 4 / 5                   &      & ~\cite{you2021benchmarking, ocasio2019scrna}
\\
percent of mt reads     & 3 / 4 / 5                    &      & ~\cite{you2021benchmarking, ocasio2019scrna}
\\
percent of hb reads     & 3 / 4 / 5                    &        & ~\cite{oelen2022single}
\\
percent of rb reads     & 3 / 4 / 5                    &         & ~\cite{subramanian2022biology}
\\
Is doublet                 & True / False                 &         & ~\cite{wolock2019scrublet}
\\ \bottomrule[1.5pt]
\end{tabular}%
}
}
\caption{Summary of Quality Control}
\label{tab:caption}
\end{table}
